SASA: A Scalable and Automatic Stencil Acceleration Framework for Optimized Hybrid Spatial and Temporal Parallelism on HBM-based FPGAs

Stencil computation is one of the fundamental computing patterns in many application domains such as scientific computing and image processing. While there are promising studies that accelerate stencils on FPGAs, there lacks an automated acceleration framework to systematically explore both spatial and temporal parallelisms for iterative stencils that could be either computation-bound or memory-bound. In this paper, we present SASA, a scalable and automatic stencil acceleration framework on modern HBM-based FPGAs. SASA takes the high-level stencil DSL and FPGA platform as inputs, automatically exploits the best spatial and temporal parallelism configuration based on our accurate analytical model, and generates the optimized FPGA design with the best parallelism configuration in TAPA high-level synthesis C++ as well as its corresponding host code. Compared to state-of-the-art automatic stencil acceleration framework SODA that only exploits temporal parallelism, SASA achieves an average speedup of 3.74x and up to 15.73x speedup on the HBM-based Xilinx Alveo U280 FPGA board for a wide range of stencil kernels.

==> Sections/ack.tex <==
\section*{Acknowledgements}
We acknowledge the support from NSERC Discovery Grant RGPIN-2019-04613, DGECR-2019-00120, Alliance Grant ALLRP-552042-2020, CWSE PDF (470957), and RGPIN341516; Canada Foundation for Innovation John R. Evans Leaders Fund and British Columbia Knowledge Dev. Fund; Simon Fraser University New Faculty Start-up Grant; Huawei, Xilinx, and Nvidia.

==> Sections/bg_full.tex <==
%\vspace{-0.1in}
\section{Background and Related Work} \label{sec:background}

\subsection{Stencil Computation}

Stencil computation usually operates on a multidimensional array and updates each data cell using its neighbor cells in a fixed pattern. Listing~\ref{list:example} shows an example of the JACOBI2D stencil kernel, which is a 5-point, 2-dimensional stencil that computes and updates each data cell (i.e., $output[i][j]$) with its five neighbor cells. In practice, such a stencil kernel will be executed multiple iterations; in the next iteration, the output array from the previous iteration becomes the input, while the input array from the previous iteration becomes the output. As discussed earlier in the introduction, depending on the stencil operations and the number of iterations, the stencil kernel could be either computation-bound or memory-bound, and would require a different parallelism optimization.

\begin{lstlisting}[frame=single, numbers=none,  basicstyle=\small, caption = A 5-point stencil JACOBI2D kernel, label={list:example}, language=C++]
void jacobi2d (float input[R][C], float output[R][C]) {
  for (int i = 1; i < R - 1; ++i)
    for (int j = 1; j < C - 1; ++j)
      output[i][j] = (input[i][j-1] + input[i-1][j] + input[i][j]
                   + input[i][j+1] + input[i+1][j]) / 5;
}
\end{lstlisting}



\subsection{FPGA Acceleration for Stencil Computation} \label{subsec:fpga-acc}

% Table to show the feature coverage in previous work and ours
\begin{table}[!htb]
\vspace{-0.05in}
\caption{Comparison of stencil acceleration frameworks}
\vspace{-0.05in}
\label{tbl:feature-compare}
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} &
  \begin{tabular}[c]{@{}c@{}}Multi-PE\\ parallelism\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Pre-processing\\ free\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Automatic\\ optimization\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Processing\\ style\end{tabular} \\ \hline
~\cite{TemporalICCAD17}          & temporal & yes & yes & streaming\\ \hline
~\cite{ShuoWangDAC17}            & hybrid   & yes & no & data tiling \\ \hline
~\cite{SpatialTemporyBlocking18} & hybrid   & no  & no  & streaming\\ \hline
~\cite{StencilHBM20}             & hybrid   & no  & no  & streaming\\ \hline
~\cite{SODA18}                   & temporal & yes & yes & streaming\\ \hline
Ours                             & hybrid   & yes & yes & streaming\\ \hline
\end{tabular}
\end{table}

Previous research efforts in FPGA-based stencil computing generally target the following aspects: 1) exploring temporal and spatial parallelisms in accelerator designs, 2) minimizing the FPGA on-chip memory usage for the stencil computation, 3) leveraging the HBM memory on modern FPGAs to further extend the spatial parallelism, and 4) facilitating automatic stencil design generation.

Various studies have explored accelerating the iterative stencil computation through various types of parallelism. 
Namely, acceleration through temporal parallelism has been well studied and explored in most previous iterative stencil kernel accelerator designs on FPGA~\cite{TemporalICCAD17, ShuoWangDAC17,  SpatialTemporyBlocking18, SODA18, HighOrderFPGAStencil18, StencilHBM20}. And designs that also explore spatial parallelism are investigated in~\cite{ShuoWangDAC17, SpatialTemporyBlocking18, HighOrderFPGAStencil18, MultiFPGAStencil19, StencilHBM20}.% Temporal parallelism
In~\cite{TemporalICCAD17}, Natale et al. designed a dataflow architecture that executes multiple stencil computing iterations as multiple temporal stages. However, it lacks exploiting the spatial parallelism during processing of a single iteration stage.
In SODA~\cite{SODA18}, Chi et al. focused on exploiting the temporal parallelism in iterative stencil acceleration and proposed a solution to minimize the reuse buffer size and leveraged microarchitectural design optimizations to also minimize the external memory access. % Spatial parallelism
In~\cite{ShuoWangDAC17},~\cite{SpatialTemporyBlocking18}, and~\cite{StencilHBM20}, designs were proposed to use multiple PEs to exploit both spatial and temporal parallelisms. However, their designs lead to a significant on-chip memory usage overhead. This is because the streaming-based designs in~\cite{SpatialTemporyBlocking18} and~\cite{StencilHBM20} require the reuse buffers to be replicated across multiple PEs; and the design in~\cite{ShuoWangDAC17} needs to load multiple tiles of data on chip for its PEs to execute in parallel. 

In terms of minimizing the FPGA on-chip memory usage for the stencil computation, a sliding-window design is used in~\cite{SlidingWindow} that requires maintaining only a small on-chip buffer to reduce the BRAM usage, but introduces additional off-chip communication overhead.
Another graph-theory based implementation proposed in~\cite{GraphBasedFPGA18} can derive the minimum memory partition factor and use the minimum number of on-chip memory banks, but such a design targets only a limited set of stencil kernels.

To further exploit the spatial parallelism by leveraging the HBM memory on modern FPGAs,~\cite{SpatialTemporyBlocking18} and~\cite{StencilHBM20} explored utilizing multiple memory banks of an HBM in their single PE design. However, their implementations require data pre-processing on the host CPU side to allow the parallel memory access and to exploit the efficient burst access from the FPGA off-chip HBM memory. This would introduce additional latency between stencil iterations, but was not quantitatively evaluated and discussed in the work. 
To facilitate the automatic design generation and mitigate the long design exploration process, previous work have developed high-level DSL to generate the stencil computing designs on FPGAs~\cite{SODA18, DSL1, DSL2, DSL3}, but only in~\cite{SODA18} did it also support an automatic design exploration and optimization based on accurate analytical performance models. An automatic design optimization framework is also proposed in~\cite{ShuoWangDAC17}, but its architecture is template-based instead of generated from a high-level DSL.

The goal of this paper is to develop an automatic stencil acceleration framework,~\toolName, to incorporate the all the features as summarized in Table~\ref{tbl:feature-compare}. 
First, ~\toolName is a streaming-based design similar to SODA~\cite{SODA18} for achieving the optimal data reuse, and additionally include coalesced reuse buffers to further reduce resource utilization on FPGAs.
In addition,~\toolName leverages a hybrid multi-PE design architecture exploiting both spatial and temporal parallelisms. This is because when the stencil iteration number is high and computation intensity is high (i.e., computation-bound), the major performance improvement comes from the parallelized the memory access and data computation of each stencil iteration, as the spatial parallelism can efficiently accelerate the computation of the design. On the contrary, for the memory-bound stencil kernels, the performance gain comes from the data reuse across processing multiple consecutive stencil iterations in a pipelined fashion on FPGA.
Furthermore,~\toolName utilizes the HBM memory on modern FPGAs, yet unlike previous HBM-based stencil designs, our tool does not require any data pre-processing on the CPU host side.
And lastly, in terms of design automation,~\toolName enables end-users to define their stencil operations through DSL and then automatically optimize and generate the accelerator design based an analytically performance model.

% \subsection{Problem Formulation}
% % Talk about the problem that we try to solve
% % APPLICATION
% % Iterative Stencil
% % Memory bound - Iteration num
% % Hardware
% % HBM & multi-die
% % Automatic flow
% Bottleneck of stencil algorithm is decided by both algorithm complexity and iteration number. Iterative stencil algorithm shown in Listing~\ref{list:example} is relatively simple with small operation number on each cell computation. In other words, operation intensity of algorithm in Listing~\ref{list:example} is small. When iteration number is relatively small, such applications will be memory-bound. However, when iteration number is sufficiently large, the operation intensity will be sufficiently high, which makes stencil applications computation-bound. In this case, all optimizations will be limited by the available hardware resource. Figure~\ref{fig:intensityA} shows the computation intensity of all benchmarks presented in ascending order with operation number per byte. Figure~\ref{fig:intensityB} shows intensity of one benchmark, JACOBI2D, across different iteration number as example. 

% % \begin{figure}[h]
% %     \centerline{
% %     \includegraphics[width=0.5\textwidth]{Fig/Intensity.pdf}}
% %     \vspace{-0.05in}
% %     \caption{Computation Intensity Comparison}
% %     \label{fig:intensity}
% % \end{figure}
% % \begin{figure}[!t]
% %     \centering
% %     \begin{subfigure}[b]{0.45\textwidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{Fig/IntensityB.pdf}
% %         \caption{Computation intensity of different stencil kernels with the number of iterations = 2}
% %         \label{fig:intensityA}
% %     \end{subfigure}
% %     \begin{subfigure}[b]{0.45\textwidth}
% %         \centering
% %         \includegraphics[width=\textwidth]{Fig/IntensityA.pdf}
% %         \caption{Computation intensity of the JACOBI2D stencil kernel with different numbers of iterations}
% %         \label{fig:intensityB}
% %     \end{subfigure}
% %     \caption{Computation intensity comparison for different stencil kernels and different numbers of iterations}
% %     \label{fig:intensity}
% % \end{figure}

% To increase the data reuse, multiple processing elements(PEs) can be combined together where each PE is called one stage. Each stage will work on one iteration and store its output in the on-chip memory which will be used as the input of the next stage. Such optimization is called temporal parallelism. 

% Most previous designs were limited by the number of off-chip memory ports. With restricted external memory bandwidth, they need to split input data into multiple blocks or tiles processing large input size and all blocks or tiles are handled in sequence.
% By utilizing HBM on modern FPGA, each PE can compute on one tile in parallel and further gain advantage from reduced halo region. This optimization is called spatial parallelism.

% To choose a proper stencil accelerator design among various optimization options, we need to incorporate multiple factors like the number of iterations, hardware platform constraints, etc.
% Besides, such workflow can be automatized to lighten the burden of writing efficient FPGA code and manual design space exploration.


==> Sections/related.tex <==
%\vspace{-0.1in}
\section{Related Work}\label{sec:related}



==> Sections/revision.tex <==
% Dear Reviewers,
\noindent Dear Editor and Reviewers,

We would like to thank you for your hard work and insightful comments. Based on the reviewers' requests and comments, we have made many changes to improve the quality of our paper in this revision. Our response, including details of the changes made, is included inline below (\rev{highlighted in blue}). Those major changes are also highlighted in the submitted paper. Two additional PDFs are included as part of this updated submission: one, with simply the new version of the text, and the other, where all text changes have been highlighted.

\textbf{Major Framework Change:}

We would like to mention one major change in our SASA framework here: with the help of Licheng Guo and Yuze Chi from UCLA, we have integrated their open source TAPA/AutoBridge framework [5,14] into our SASA framework to address the timing closure issue and conduct a fairer comparison between different parallelism implementations. The TAPA/AutoBridge framework has three major advantages. First, it supports easier programming of task-parallel dataflow programs in C++, without the need of the more complex OpenCL approach (using multiple OpenCL kernels) to support task parallelism. Our SASA code generator automatically converts the stencil DSL to the TAPA HLS and host code. One thing to note is that in TAPA HLS, there is only one FPGA kernel; so we have renamed “kernel-to-kernel streaming” to “border streaming” in the revision.  Second, it replaces the resource-inefficient AXI interface with a lightweight streaming interface to access off-chip memory. The standard AXI interface always buffers data in BRAM and consumes a significant amount of resources on the bottom die of the HBM-based U280 FPGA (with multiple AXI interfaces), which often causes place-and-route congestion and timing violation  on the bottom die. With the lightweight streaming interfaces, it saves resources for actual computations and reduces place-and-route congestion and timing violation  on the bottom die. Third, it automatically applies coarse-grained floorplanning and pipelining optimizations to improve the timing closure for dataflow programs, and can often greatly improve the design build success rate and the final design frequency. With this integration, we have rerun our experiments with higher numbers of PEs to conduct a fairer comparison between different parallelisms. A detailed description of our framework changes is highlighted in Sec 4.3 of our paper.

We would like to add Licheng Guo and Yuze Chi as the paper co-authors in this revision, for their great efforts in helping integrate and improve the TAPA/AutoBridge framework for stencil applications. 

\noindent \textbf{Reviewer \#1:}

1.1 Tradeoff between redundant computation and border streaming (we have renamed “kernel-to-kernel streaming” to “border streaming” in the revision, as explained above.)
Response: To better evaluate the tradeoff between the redundant computation based and border streaming based spatial parallelisms (or hybrid parallelisms) in a fairer way, in this revision, we have integrated the open-source TAPA/AutoBridge framework into our SASA framework to address the timing closure issue. As a result, most redundant computation based and border streaming based spatial parallelisms (or hybrid parallelisms) can achieve the same number of PEs. Our new experimental results are highlighted in Sec 5.2 and Sec 5.3(including Figure 10 to Figure 20). Below is a summary of the results.

